sqlelf: a SQL-centric Approach to ELF Analysis

The exploration and understanding of Executable and Linkable Format (ELF) objects underpin various critical activities in computer systems, from debugging to reverse engineering. Traditional UNIX tooling like readelf, nm, and objdump have served the community reliably over the years. However, as the complexity and scale of software projects has grown, there arises a need for more intuitive, flexible, and powerful methods to investigate ELF objects. In this paper, we introduce sqlelf, an innovative tool that empowers users to probe ELF objects through the expressive power of SQL. By modeling ELF objects as relational databases, sqlelf offers the following advantages over conventional methods. Our evaluations demonstrate that sqlelf not only provides more nuanced and comprehensive insights into ELF objects but also significantly reduces the effort and time traditionally required for ELF exploration tasks

==> text/acknowledgements.tex <==
\section*{Acknowledgements}

This work was in part supported by the National Science Foundation under Cooperative Agreement OAC-1836650, by the US Department of Energy ASCR DE-NA0003525 (FWP 20-023266, subcontract with Sandia National Labs), and by the Center for Research in Open Source Software (\url{https://cross.ucsc.edu}).  This work was performed under the auspices of the U.S. Department of Energy by Lawrence Livermore National Laboratory under contract DE-AC52-07NA27344. Lawrence Livermore National Security, LLC.


==> text/evaluation-unused.tex <==
\section{Evaluation}
\arq{Update for consistency with evaluation questions}
\label{sec:evaluation}

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\columnwidth]{images/benchmark_symbol_size.pdf}
    \caption{\sys vs. readelf in discovering number of symbols}
    \label{fig:benchmark-symbol-size}
\end{figure}

Python was chosen as the development language for its ease of use, iterative speed, and widespread audience. Unsurprisingly however, the choice of language comes at a performance cost when compared to the traditional tools (\verb`readelf` or \verb`objdump`) which are written in C/C++. Since any table may be a bottleneck for \sys, we can use the single table \verb`ELF_SYMBOLS` as a proxy for the performance. Additionally, by offering a SQL frontend, the performance is also affected by the complexity of the task and query. To ground us in some ground-truths, we chose to look at a straightforward query that can be easily replicated using \verb`readelf` and \verb`wc` which is to count the number of symbols within an ELF file. We benchmarked the contrasting pipelines by generating executable ELF files with the desired number of symbols. Although consistently slower than its counterparts, the tool performs acceptably well for ELF files with up to 10000 symbols achieving sub-second execution times. As the number of symbols begins to approach or go beyond $1\mathrm{e}{5}$ the latency is exceedingly slow as depicted in Figure~\ref{fig:benchmark-symbol-size}. We have added support in the tool to export the in-memory SQLite database to a file on disk, effectively memoizing the creation of the database which can be used to mitigate this performance penalty. Performing the queries against the memoized database using the native SQLite client consistently achieves speeds that outperform the \verb`readelf` pipeline.

We were interested in understanding how realistic are binaries that exceed $1\mathrm{e}{4}$ symbols. We audited roughly 1600 ELF files (\verb`/bin`, \verb`/usr/bin` and \verb`/lib/x86_64-linux-gnu`) on a fresh Ubuntu 22.04 installation and failed to find a binary whose symbol count surpassed 30000 shown in Figure~\ref{fig:ubuntu-symbol-histogram}. The largest ELF file in terms of symbol was the tool \verb`lto-dump` with 21127 symbols. Nearly all installed binaries on a Debian based machine are dynamically-linked which would reduce the maximum number of symbols per any given file. At Google, most binaries are statically-linked and it is not uncommon to find extremely large binaries (>2GiB). It's common for such binaries to have well over 1 million ($1\mathrm{e}{6}$) symbols. With so many symbols, even generating the memoized database can be an overly time-consuming step. % Add back in for future work section % We outline some improvements that are underway and additional opportunities in Section~\ref{sec:future-work} to scale sqlelf to these massively large binaries.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{images/symbols_ubuntu_histogram.pdf}
    \caption{Number of symbols per executable on a typical Ubuntu installation}
    \label{fig:ubuntu-symbol-histogram}
\end{figure}

==> text/future_work.tex <==
\section{Future Work}\label{sec:future-work}

% TODO(fmzakari) this is just GPT barf at the moment

We are excited by the new opportunities available for analysis with the power of SQL however we see continued opportunity for improvement and refinement in the domain space which we are actively exploring.

One of the structural enhancements under consideration involves a transition to C/C++ for the core implementation of sqlelf. While the existing Python implementation affords ease of use and rapid development, the intrinsic performance limitations, particularly pertinent when handling large ELF files such as typically found at Google or executing complex queries, necessitate this transition. Python has great support for accessing libraries written in C/C++ however the cost for traversing the virtual machine is prohibitively for large tables as the global interpreter lock (GIL) must be continuously re-acquired for each row.

The schema presented here is one nearly mirroring the ELF format itself, largely to demonstrate that the two could be interchanged in any codebase leveraging either. We are looking at supporting modifications back to the underlying file done via SQL statements. The ELF file format is intricate and compact, following a precise structure vital for the correct operation of executables and shared libraries. If necessary, a hex editor can be used to make alterations, assuming the user possesses precise knowledge regarding the specific segment of the ELF file that requires modification. It's crucial to exercise caution during this process, as errors can easily occur. Conversely, using sqelf in conjunction with a declarative language will make it more straightforward to modify the file by adding, updating, or creating new entries in the respective tables. Finally, we are continuing to refine the SQL schema to facilitate more complex spectrum of queries.

A more contemplative work we are assessing is whether there is a need for the ELF file itself and whether Linux, loaders and linkers could natively work with the SQLite database itself. This is a much more substantial change to the landscape however unlocks a myriad of possibilities, simplifying interactions and enabling novel uses of database ACID properties for binary executions. For instance, if every binary was a database and started within a transaction, we imagine we replacing \verb`LD_PRELOAD` with an \verb`UPDATE` statement to modify the desired symbols. The work to introduce sqlelf into musl's dynamic loader was an entry point into this work. We are also looking at leveraging the LLVM toolchain to assess the feasibility of using SQLite in the compilation process itself.


